Contrast-Informed Augmentation and Domain-Adversarial Training for Adult-to-Neonatal MR Reconstruction Generalization

Purpose: To investigate whether contrast-informed data augmentation and domain-adversarial training improve the adult-to-neonatal generalization of the E2E-VarNet. Methods: Three training regimes were investigated: (1) adult-only training with unaugmented adult data, (2) mixed training with paired unaugmented and neonatal-informed augmented adult data, and (3) mixed training with a domain-adversarial objective. Models were trained on retrospectively undersampled multi-coil adult T2-weighted brain MR data and evaluated on neonatal and adult test data at acceleration factors $R=4$ and $R=8$ using quantitative metrics and qualitative evaluation. Feature analyses assessed whether domain-adversarial training altered the latent representations of unaugmented adult, augmented adult, and neonatal test samples. Results: Mixed training (Mixed) and mixed domain-adversarial training (Mixed-DAT) outperformed unaugmented adult-only training (Unaug-Only) when evaluated on neonatal data. At R=4, Mixed-DAT achieved the best performance (SSIM = 0.924 +/- 0.027, PSNR = 33.98 +/- 1.15 dB). At R=8, Mixed-DAT performed best when measured using SSIM (0.848 +/- 0.031 vs. 0.766 +/- 0.037 for Unaug-Only and 0.814 +/- 0.035 for Mixed) and Mixed performed best when measured using PSNR (29.56 +/- 0.83 dB vs. 26.26 +/- 0.78 dB for Unaug-Only and 29.43 +/- 0.83 dB for Mixed-DAT). Qualitative assessment of t-SNE plots suggested that Mixed-DAT increased the overlap among the latent representations of the unaugmented adult, augmented adult, and neonatal test data. Conclusion: Contrast-informed augmentation and domain-adversarial training improved adult-to-neonatal generalization of deep learning-based MR reconstruction. These findings suggest that contrast-informed data augmentation combined with adversarial training may improve robustness to domain shift in undersampled neonatal MR reconstruction.

==> results_table_adult.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lcccc}
        \toprule
        & R4 SSIM & R4 PSNR & R8 SSIM & R8 PSNR \\
        \midrule
        Adult-only      & 0.938 $\pm$ 0.034 & 38.03 $\pm$ 2.43 & \textbf{0.917 $\pm$ 0.035} & 34.11 $\pm$ 1.55 \\
        Mixed           & \textbf{0.940 $\pm$ 0.032} & 38.37 $\pm$ 2.32 & 0.916 $\pm$ 0.038 & \textbf{34.28 $\pm$ 2.00} \\
        Mixed with DAT  & \textbf{0.940 $\pm$ 0.034} & \textbf{38.44 $\pm$ 2.55} & 0.915 $\pm$ 0.038 & 34.01 $\pm$ 2.17 \\
    \end{tabular}
    \caption{Summary of average performance measure per volume (mean $\pm$ standard deviation) for each experiment on the adult test set.}
    \label{tab:results_table_adult}
\end{table}

==> results_table_neonatal.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lcccc}
        \toprule
        & R4 SSIM & R4 PSNR & R8 SSIM & R8 PSNR \\
        \midrule
        Adult-only      & 0.866 $\pm$ 0.032 & 32.68 $\pm$ 1.18 & 0.766 $\pm$ 0.037 & 26.26 $\pm$ 0.78 \\
        Mixed           & \textbf{0.895 $\pm$ 0.027} & 33.49 $\pm$ 1.14 & 0.814 $\pm$ 0.035 & 29.56 $\pm$ 0.83 \\
        Mixed with DAT  & 0.891 $\pm$ 0.030 & \textbf{33.58 $\pm$ 1.19} & \textbf{0.836 $\pm$ 0.032} & \textbf{29.81 $\pm$ 0.87} \\
    \end{tabular}
    \caption{Summary of average performance measure per volume (mean $\pm$ standard deviation) for each experiment on the neonatal test set.}
    \label{tab:results_table_neonatal}
\end{table}
